FLSea: Underwater Visual-Inertial and Stereo-Vision Forward-Looking Datasets

Visibility underwater is challenging, and degrades as the distance between the subject and camera increases, making vision tasks in the forward-looking direction more difficult. We have collected underwater forward-looking stereo-vision and visual-inertial image sets in the Mediterranean and Red Sea. To our knowledge there are no other public datasets in the underwater environment acquired with this camera-sensor orientation published with ground-truth. These datasets are critical for the development of several underwater applications, including obstacle avoidance, visual odometry, 3D tracking, Simultaneous Localization and Mapping (SLAM) and depth estimation. The stereo datasets include synchronized stereo images in dynamic underwater environments with objects of known-size. The visual-inertial datasets contain monocular images and IMU measurements, aligned with millisecond resolution timestamps and objects of known size which were placed in the scene. Both sensor configurations allow for scale estimation, with the calibrated baseline in the stereo setup and the IMU in the visual-inertial setup. Ground truth depth maps were created offline for both dataset types using photogrammetry. The ground truth is validated with multiple known measurements placed throughout the imaged environment. There are 5 stereo and 8 visual-inertial datasets in total, each containing thousands of images, with a range of different underwater visibility and ambient light conditions, natural and man-made structures and dynamic camera motions. The forward-looking orientation of the camera makes these datasets unique and ideal for testing underwater obstacle-avoidance algorithms and for navigation close to the seafloor in dynamic environments. With our datasets, we hope to encourage the advancement of autonomous functionality for underwater vehicles in dynamic and/or shallow water environments.

==> dataset_table_w_measurements.tex <==
\begin{table*}[!h]
\small\sf
\caption{Datasets. \label{datasets}}
\begin{tabular}{p{2cm} p{3.5cm} p{3cm} p{3.5cm} p{3cm}} %{0.8\textwidth}
\toprule
\multicolumn{5}{c}{Visual-Inertial}\\
\midrule
 \textbf{Location}& \textbf{Dataset name} & \textbf{Image number} & \textbf{Trajectory length (m)} & \textbf{Area (m\textsuperscript{2})} \\
 \multirow{4}{*}{Canyons} & U Canyon & 2895 & 46.92 & 89\\
 & Flatiron & 2475 & 46.21 & 67\\
 & Horse Canyon & 2230 & 84.69 & 45\\
 & Tiny Canyon & 1012 & 52.99 & 10 \\
 \bottomrule
 \multirow{8}{*}{Red Sea} & Northeast Path & 2593 & & 210 \\ 
 & Landward Path & 1204 & & 122\\
 & Dice Path & 1428 & & 72\\
 & Pier Path & 1695 & & 94\\
 & Coral Table Loop & 1017 & & 73\\
 & Cross Pyramid Loop & 1652 & & 102\\
 & Big Dice Loop & 3159 & & 412\\
 & Sub Pier & 1091 & & 48\\
\bottomrule
\end{tabular}\\[10pt]
\begin{tabular}{p{2cm} p{3.5cm} p{3cm} p{3.5cm} p{3cm}}
\toprule
\multicolumn{5}{c}{Stereo} \\
\midrule
 \textbf{Location}& \textbf{Dataset name} & \textbf{Image number} & \textbf{Trajectory length (m)} & \textbf{Area (m\textsuperscript{2})} \\
 \multirow{2}{*}{Canyons} & Canyon 1 & 7606 L/R pairs & &\\
 & Canyon 2 & 2363 L/R pairs & & \\
\multirow{2}{*}{Shallow} & Flats & 2702 L/R pairs & &\\
& Rock Garden 1 & 5688 L/R pairs & & \\
& Rock Garden 2 & 1238 L/R pairs & & \\
\bottomrule
\end{tabular}\\[10pt]
\end{table*}


\begin{table}[H]
\small\sf\centering
\caption{U Canyon dataset.\label{u_canyon}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & U Canyon\\
Date & June 10, 2021\\
Time & 08:43\\
Max site depth & 6~m\\
Approx. trajectory length & 47~m\\
Approx. area & 90~m\textsuperscript{2}\\
Set duration & 4' 50''\\
Number of frames & 2895\\
Frame rate & 10~fps\\
IMU rate & 20~Hz (interpolated to 100~Hz available)\\
Site description & Half in canyon, half out, loops around area filled with large rocks. Some over exposure in the images.\\
Known objects & Scale cards, meter tape and April tag board.\\
Bottom type & Sandy, with large rocks\\
Visual disturbances & Turbidity, dynamic objects, caustics\\
Dynamic objects & small fish, jellyfish\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Flatiron dataset.\label{flatiron}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Flatiron\\
Date & June 10, 2021\\
Time & 09:00\\
Max site depth & 4~m\\
Approx. trajectory length & \\
Approx. area & 67~m\textsuperscript{2}\\
Set duration & 4' 08''\\
Number of frames & 2475\\
Frame rate & 10~fps\\
IMU rate & 20~Hz (interpolated to 100~Hz available)\\
Site description & Flat open area, many large rocks.\\
Known objects & Scale cards, meter tape and April tag board.\\
Bottom type & Sandy, with large rocks\\
Visual disturbances & Turbidity, dynamic objects, caustics\\
Dynamic objects & small fish, jellyfish\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Horse Canyon dataset.\label{horse_canyon}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Horse Canyon\\
Date & June 10, 2021\\
Time & 11:58\\
Max site depth & 7~m\\
Approx. trajectory length & \\
Approx. area & 45~m\textsuperscript{2}\\
Set duration & 3' 43''\\
Number of frames & 2230\\
Frame rate & 10~fps\\
IMU rate & 20~Hz (interpolated to 100~Hz available)\\
Site description & Back and forth through canyon with 3d structure.\\
Known objects & Scale cards, meter tape and April tag board.\\
Bottom type & Sandy, with large rocks\\
Visual disturbances & Turbidity, dynamic objects, caustics, low light\\
Dynamic objects & small fish\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Tiny Canyon dataset.\label{tiny_canyon}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Tiny Canyon\\
Date & June 10, 2021\\
Time & 12:16\\
Max site depth & 5~m\\
Approx. trajectory length & \\
Approx. area & 10~m\textsuperscript{2}\\
Set duration & 1' 42''\\
Number of frames & 1012\\
Frame rate & 10~fps\\
IMU rate & 20~Hz (interpolated to 100~Hz available)\\
Site description & Pass through very small canyon, mostly low light, but includes change from low to normal ambient light at the end.\\
Known objects & Scale cards, meter tape and April tag board.\\
Bottom type & Sandy, with large rocks\\
Visual disturbances & Turbidity, dynamic objects, caustics, low light\\
Dynamic objects & small fish\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Northeast Path.\label{northeast_path}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Northeast Path\\
Date & 08:31\\
Max site depth & 6~m\\
Approx. trajectory length & \\
Approx. area & 210~m\textsuperscript{2}\\
Set duration & 4' 20''\\
Number of frames & 2593\\
Frame rate & 10~fps\\
IMU rate & 100~Hz\\
Site description & Back and forth along path with some 3D structure, man-made and natural.\\
Known objects & Scale cards, meter tape, April tag board and pier.\\
Bottom type & Rocky, some coral\\
Visual disturbances & Turbidity, dynamic objects, caustics\\
Dynamic objects & small fish\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Landward Path.\label{landward_path}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Landward Path\\
Date & 09:01\\
Max site depth & 6~m\\
Approx. trajectory length & \\
Approx. area & 122~m\textsuperscript{2}\\
Set duration & 2'\\
Number of frames & 1204\\
Frame rate & 10~fps\\
IMU rate & 100~Hz\\
Site description & Back and forth along transect with some 3D structure, man-made (pier, pipes) and natural (rocks, coral).\\
Known objects & Scale cards, meter tape, April tag board and pier.\\
Bottom type & Rocky, some coral\\
Visual disturbances & Turbidity, dynamic objects, caustics\\
Dynamic objects & small fish\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Dice Path.\label{dice_path}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Dice Path\\
Date & 13:12\\
Max site depth & 6~m\\
Approx. trajectory length & \\
Approx. area & 72~m\textsuperscript{2}\\
Set duration & 2' 22''\\
Number of frames & 1428\\
Frame rate & 10~fps\\
IMU rate & 100~Hz\\
Site description & Path on flat open area with some 3D structure, man-made (``dice,'' pier, pipes) and natural (rocks, coral).\\
Known objects & Scale cards, meter tape, April tag board and pier.\\
Bottom type & Rocky\\
Visual disturbances & Turbidity, dynamic objects, caustics\\
Dynamic objects & small fish\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Pier Path.\label{pier_path}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Pier Path\\
Date & 13:45\\
Max site depth & 4~m\\
Approx. trajectory length & \\
Approx. area & 94~m\textsuperscript{2}\\
Set duration & 2' 49''\\
Number of frames & 1695\\
Frame rate & 10~fps\\
IMU rate & 100~Hz\\
Site description & Path through flat open area towards pier, with man-made (pier, pipes) and natural structure (rocks, coral).\\
Known objects & Scale cards, meter tape, April tag board and pier.\\
Bottom type & Rocky\\
Visual disturbances & Turbidity, dynamic objects\\
Dynamic objects & small fish\\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[H]
\small\sf\centering
\caption{Coral Table Loop.\label{coral_table_loop}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Coral Table Loop\\
Date & 07:58\\
Max site depth & 8~m\\
Approx. trajectory length & \\
Approx. area & 73~m\textsuperscript{2}\\
Set duration & 1' 41''\\
Number of frames & 1017\\
Frame rate & 10~fps\\
IMU rate & 100~Hz\\
Site description & Path through flat open area with man-made structure (coral tables) and minimal natural structure.\\
Known objects & Scale cards, meter tape and April tag board.\\
Bottom type & Rocky\\
Visual disturbances & Turbidity, dynamic objects\\
Dynamic objects & small fish\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Cross Pyramid Loop.\label{cross_pyramid_loop}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Cross Pyramid Loop\\
Date & 08:13\\
Max site depth & 8~m\\
Approx. trajectory length & \\
Approx. area & 102~m\textsuperscript{2}\\
Set duration & 2' 45''\\
Number of frames & 1652\\
Frame rate & 10~fps\\
IMU rate & 100~Hz\\
Site description & Path through flat open area next to a coral table pyramid and minimal natural structure.\\
Known objects & Scale cards, meter tape and April tag board.\\
Bottom type & Rocky\\
Visual disturbances & Turbidity, dynamic objects\\
Dynamic objects & small fish\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Big Dice Loop.\label{big_dice_loop}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Big Dice Loop\\
Date & 09:26\\
Max site depth & 6~m\\
Approx. trajectory length & \\
Approx. area & 412~m\textsuperscript{2}\\
Set duration & 5' 15''\\
Number of frames & 3159\\
Frame rate & 10~fps\\
IMU rate & 100~Hz\\
Site description & Path on flat open area with some 3D structure, man-made (``dice,'' pier, pipes) and natural (rocks, coral).\\
Known objects & Scale cards, meter tape, April tag board and pier.\\
Bottom type & Rocky\\
Visual disturbances & Turbidity, dynamic objects, caustics\\
Dynamic objects & small fish, diver\\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\small\sf\centering
\caption{Sub Pier.\label{sub_pier}}
\begin{tabular}{p{3.5cm} p{4cm}} %{0.8\textwidth}
\toprule
Site name & Sub Pier\\
Date & 09:57\\
Max site depth & 4~m\\
Approx. trajectory length & \\
Approx. area & 48~m\textsuperscript{2}\\
Set duration & 1' 49''\\
Number of frames & 1091\\
Frame rate & 10~fps\\
IMU rate & 100~Hz\\
Site description & Path underneath pier, shallow water, lots of fish, caustics and ambient light changes.\\
Known objects & Scale cards, meter tape, April tag board and pier.\\
Bottom type & Rocky\\
Visual disturbances & Turbidity, dynamic objects, caustics\\
Dynamic objects & small fish\\
\bottomrule
\end{tabular}
\end{table}
